Enabling Experimental Impulse-Based Substructuring through Time Domain Deconvolution and Downsampling

Dynamic substructuring, especially the frequency-based variant (FBS) using frequency response functions (FRF), is gaining in popularity and importance, with countless successful applications, both numerically and experimentally. One drawback, however, is found when the responses to shocks are determined. Numerically, this might be especially expensive when a huge number of high-frequency modes have to be accounted for to correctly predict response amplitudes to shocks. In all cases, the initial response predicted using frequency-based substructuring might be erroneous, due to the forced periodization of the Fourier transform. This drawback can be eliminated by completely avoiding the frequency domain and remaining in the time domain, using the impulse-based substructuring method (IBS), which utilizes impulse response functions (IRF). While this method has already been utilized successfully for numerical test cases, none of the attempted experimental applications were successful. In this paper, an experimental application of IBS to rods considered as one-dimensional is tested in the context of shock analysis, with the goal of correctly predicting the maximum driving point response peak. The challenges related to experimental IBS applications are discussed and an improvement attempt is made by limiting the frequency content considered through low-pass filtering and downsampling. The combination of a purely time domain based estimation procedure for the IRFs and the application of low-pass filtering with downsampling to the measured responses enabled a correct prediction of the initial shock responses of the rods with IBS experimentally, using displacements, velocities and accelerations.

==> source/numerical.tex <==
% !TeX spellcheck = en_US
\section{Numerical Pre-Study of Impulse Response Function Identification Methods}

\subsection{Utilized Numerical Model}

\begin{figure}[ht]
	\centering
	\def\svgwidth{0.7\textwidth}
	\input{figures/numerical/1D_bar_system_sketch.pdf_tex}
	\caption{Overview of geometry and coordinates of the 1D rods considered as test pieces}
	\label{fig:1D_bar_overview_numeric}
\end{figure}



\subsection{Methodology}

\begin{equation}
	I_P(t)=\dfrac{F_{\text{imp}}}{2}\cdot\left(1-\cos\left(2\pi\dfrac{t}{T_{\text{imp}}}\right)\right)\quad\text{for}\quad 0\leqslant t\leqslant T_{\text{imp}} \label{eq:ImperfectImpulse}
\end{equation}

\subsection{Results}

\subsubsection{Frequency Domain Identification}

\subsubsection{Time Domain Identification}
